Regret Minimization with Noisy Observations

In a typical optimization problem, the task is to pick one of a number of options with the lowest cost or the highest value. In practice, these cost/value quantities often come through processes such as measurement or machine learning, which are noisy, with quantifiable noise distributions. To take these noise distributions into account, one approach is to assume a prior for the values, use it to build a posterior, and then apply standard stochastic optimization to pick a solution. However, in many practical applications, such prior distributions may not be available. In this paper, we study such scenarios using a regret minimization model. In our model, the task is to pick the highest one out of $n$ values. The values are unknown and chosen by an adversary, but can be observed through noisy channels, where additive noises are stochastically drawn from known distributions. The goal is to minimize the regret of our selection, defined as the expected difference between the highest and the selected value on the worst-case choices of values. We show that the na\"ive algorithm of picking the highest observed value has regret arbitrarily worse than the optimum, even when $n = 2$ and the noises are unbiased in expectation. On the other hand, we propose an algorithm which gives a constant-approximation to the optimal regret for any $n$. Our algorithm is conceptually simple, computationally efficient, and requires only minimal knowledge of the noise distributions.

==> note.tex <==

\section{Setting}
We are deciding whether or not to take an item. The item has value $v \in \mathbb{R}$, which is unknown to us. However, we can see the observed value $s = v + a$, where $a \in A$ is a noise. We know the noise distribution $A$. Without loss of generality, we assume $\E[A] = 0$. We also assume $A$ is continuous (maybe also bounded or something).

We need to design an algorithm $\alg$ that decides whether to take the item upon observing $s$. Let $\alg(s)$ be its output when the input is $s$. $\alg(s) = 1$ means it takes the item and $\alg(s) = 0$ means otherwise. We need to minimize its regret over value set $V$:
\[
\reg_V(\alg) := \max\left(\sup_{v > 0, v \in V} \left(v \cdot \Pr_{a \sim A}[\alg(v + a) = 0]\right), \ \sup_{v < 0, v \in V} \left((-v) \cdot \Pr_{a \sim A}[\alg(v + a) = 1]\right)\right).
\]
We shorthand $\reg_\mathbb{R}(\alg)$ as $\reg(\alg)$.

\subsection{Algorithms}
Let $\opt$ be the algorithm that minimizes the regret.

Let $\thr_\theta$ be a threshold mechanism, which states a threshold $\theta$ and outputs $\alg(s) = 1$ iff $s \geq \theta$. Let $\theta^*$ be the regret-minimizing threshold (for possible values taken from $\mathbb{R}$). (It exists since $\reg(\thr_\theta)$ is continuous in $\theta$.)

%We also use $\opt$ and $\thr_\theta$ to denote their respective regrets.

\section{The Threshold Mechanism Gives a Constant-Approximation}

\begin{lemma}
There exist values $v_1 > 0$, $v_2 < 0$, so that
\[
\inf_\theta \reg(\thr_\theta) = \inf_\theta \reg_{\{v_1, v_2\}}(\thr_\theta).
\]
Moreover,
\[
\reg_{\{v_1\}}(\thr_{\theta^*}) = \reg_{\{v_2\}}(\thr_{\theta^*}).
\]
\end{lemma}
\begin{proof}
Let $v_1 > 0$ be the value that maximizes $v \cdot \Pr_{a \sim A}[\thr_{\theta^*}(v + a) = 0]$ and $v_2 < 0$ be the value that maximizes $(-v) \cdot \Pr_{a \sim A}[\thr_{\theta^*}(v + a) = 0]$. (They exist since the functions are continuous.) We prove the lemma statement for this choice of $\{v_1, v_2\}$. The non-trivial direction is to prove
\[
\inf_\theta \reg(\thr_\theta) \leq \inf_\theta \reg_{\{v_1, v_2\}}(\thr_\theta).
\]

We have
\[
\inf_\theta \reg(\thr_\theta) = \reg(\thr_{\theta^*}) = \reg_{\{v_1, v_2\}}(\thr_{\theta^*}).
\]

Notice that $\reg_{\mathbb{R}^+}(\thr_{\theta})$ is continuously increasing in $\theta$ and $\reg_{\mathbb{R}^-}(\thr_{\theta})$ is continuously decreasing in $\theta$. In order that $\theta^*$ is the optimal threshold, we must have $\reg_{\{v_1\}}(\thr_{\theta^*}) = \reg_{\{v_2\}}(\thr_{\theta^*})$. Therefore, we only need to prove
\[
\min\left((\reg_{\{v_1\}}(\thr_{\theta^*}), \reg_{\{v_2\}}(\thr_{\theta^*})\right) \leq \inf_\theta \reg_{\{v_1, v_2\}}(\thr_\theta).
\]

This is true since if $\theta > \theta^*$, then $\reg_{\{v_1, v_2\}}(\thr_\theta) \geq \reg_{\{v_1\}}(\thr_\theta) \geq \reg_{\{v_1\}}(\thr_{\theta^*})$; and if $\theta < \theta^*$ then we have the symmetric argument.
\end{proof}

\begin{lemma}
For any $\lambda > 1$, $\Pr[a < \theta^* - \lambda \cdot v_1 \mid a < \theta^* - v_1] \leq \frac{1}{\lambda}$. Similarly, for any $\lambda > 1$, $\Pr[a > \theta^* - \lambda \cdot v_2 \mid a > \theta^* - v_2] \leq \frac{1}{\lambda}$. 
\end{lemma}
\begin{proof}
We prove the first statement and a similar argument works for the second.

We know
\[
\reg_{\{v_1\}}(\thr_{\theta^*}) \geq \reg_{\{\lambda \cdot v_1\}}(\thr_{\theta^*}),
\]
which is equivalent to
\[
v_1 \cdot \Pr[v_1 + a < \theta^*] \geq \lambda \cdot v_1 \cdot \Pr[\lambda \cdot v_1 + a < \theta^*].
\]
Rearranging gives the lemma statement.
\end{proof}

\begin{lemma}
Let $D$ be the uniform distribution $U[0.8v_1, 1.2v_1]$. Then the PDF
$f_{D + A}(t) \geq 0.4 \cdot \frac{1}{v_1} \cdot \Pr[a < \theta^* - v_1]$ for any $t \in [\theta^* - 0.2v_1, \theta^*]$.

Similarly, let $D'$ be the uniform distribution $U[1.2v_2, 0.8v_2]$. Then the PDF
$f_{D' + A}(t) \geq 0.4 \cdot \frac{1}{-v_2} \cdot \Pr[a > \theta^* - v_2]$ for any $t \in [\theta^*, \theta^* - 0.2v_2]$.
\end{lemma}
\begin{proof}
We prove the first statement and a similar argument works for the second.

For any $t \in [\theta^* - 0.2v_1, \theta^*]$,
\begin{align*}
f_{D + A}(t) &= \frac{1}{0.4v_1} \cdot \int_{0.8v_1}^{1.2v_1} f_A(t - q) \d q\\
&= \frac{1}{0.4v_1} \cdot \int_{t - 1.2v_1}^{t - 0.8v_1} f_A(q) \d q\\
&\geq \frac{1}{0.4v_1} \cdot \int_{\theta^* - 1.2v_1}^{\theta^* - v_1} f_A(q) \d q\\
&\geq \frac{1}{0.4v_1} \cdot \left(1 - \frac{1}{1.2}\right) \cdot \Pr[a < \theta^* - v_1]. \qedhere
\end{align*}
\end{proof}

\begin{lemma}
Assume $v_1 \leq -v_2$. Define $k := \left\lceil \frac{-v_2}{v_1} \right\rceil$. No algorithm can get better than $0.024 \cdot \reg(\thr_{\theta^*})$ regret for both of the following two cases:
\begin{enumerate}
    \item $v$ is drawn from $D_1$, which is the uniform average of the following distributions: $U[1.0v_1, 1.4v_1]$, $U[1.2v_1, 1.6v_1], \ldots$, $U[(0.8 + 0.2k)v_1, (1.2 + 0.2k)v_1]$.
    \item $v$ is drawn from $D_2 = U[1.2v_2, 0.8v_2]$.
\end{enumerate}
\end{lemma}
\begin{proof}
Fix any algorithm $\alg$. Notice that
\begin{align*}
\reg_{v \sim D_1}(\alg) \geq 1.0v_1 \cdot (-0.2v_2) \cdot \frac{1}{k} \cdot 0.4 \cdot \frac{1}{v_1} \cdot \Pr[a < \theta^* - v_1] \cdot \Pr_{s \sim U[\theta^*, \theta^* - 0.2v_2]}[\alg(s) = 0],
\end{align*}
and
\begin{align*}
\reg_{v \sim D_2}(\alg) \geq (-0.8v_2) \cdot (-0.2v_2) \cdot 0.4 \cdot \frac{1}{-v_2} \cdot \Pr[a > \theta^* - v_2] \cdot \Pr_{s \sim U[\theta^*, \theta^* - 0.2v_2]}[\alg(s) = 1]
\end{align*}
by the previous lemma.

Therefore, (letting $S := U[\theta^*, \theta^* - 0.2v_2]$)
\begin{align*}
&\reg(\alg) \geq\\
&\max \left(0.08 (-v_2) \cdot \frac{1}{k} \cdot \Pr[a < \theta^* - v_1] \cdot \Pr_{s \sim S}[\alg(s) = 0], \ 0.064 (-v_2) \cdot \Pr[a > \theta^* - v_2] \cdot \Pr_{s \sim S}[\alg(s) = 1]\right)\\
&\geq \max \left(0.04v_1 \cdot \Pr[a < \theta^* - v_1] \cdot \Pr_{s \sim S}[\alg(s) = 0], \ 0.064 (-v_2) \cdot \Pr[a > \theta^* - v_2] \cdot \Pr_{s \sim S}[\alg(s) = 1]\right)\\
&\geq \max \left(0.04 \cdot \reg(\thr_{\theta^*}) \cdot \Pr_{s \sim S}[\alg(s) = 0], \ 0.064 \cdot \reg(\thr_{\theta^*}) \cdot \Pr_{s \sim S}[\alg(s) = 1]\right)\\
&\geq 0.024 \cdot \reg(\thr_{\theta^*}). \qedhere
\end{align*}
\end{proof}

\begin{theorem}
$\reg(\thr_{\theta^*}) \leq 42 \cdot \reg(\opt)$.
\end{theorem}

\section{Two Items}
Assume the values are $v_1$ and $v_2$, the noises are $a_1$ and $a_2$, the optimal thresholds against $0$ noise are $\theta_1$ and $\theta_2$. Consider the mechanism that uses additive offsets of $\theta_1$ and $\theta_2$. Let $v_1$ and $v_2$ be the worst case values for it. Assume $v_1 > v_2$ and let $\Delta = v_1 - v_2$. We have
\begin{align*}
\reg &= (v_1 - v_2) \cdot \Pr[v_1 + a_1 - \theta_1 < v_2 + a_2 - \theta_2]\\
&= \Delta \cdot \Pr\left[\frac{\Delta}{2} + a_1 - \theta_1 < -\frac{\Delta}{2} + a_2 - \theta_2\right]\\
&\leq \Delta \cdot \left(\Pr\left[\frac{\Delta}{2} + a_1 - \theta_1 < 0\right] + \Pr\left[-\frac{\Delta}{2} + a_2 - \theta_2 > 0\right]\right)\\
&= 2 \cdot \left(\frac{\Delta}{2} \cdot \Pr\left[\frac{\Delta}{2} + a_1 - \theta_1 < 0\right] + \frac{\Delta}{2} \cdot \Pr\left[-\frac{\Delta}{2} + a_2 - \theta_2 > 0\right]\right)\\
&\leq 2 \cdot (\reg_1 + \reg_2).
\end{align*}


\section{Multi-Item Setting}
We want to show the offset mechanism gives a constant approximation in regret. Here is the proof idea:
\begin{itemize}
    \item Fix noise distributions. Consider the (approximately) worst case value input of the offset mechanism. WLOG, let $v_1 = 0$ be the maximum value.
    \item WLOG, the offset mechanism picks $v_1$ with probability $p \geq 0.5$. This is because if $p < 0.5$, then we can uniformly decrease $v_2, \ldots, v_n$, until $p = 0.5$. The regret won't decrease by more than a factor of $2$.
    \item This means for each value from $v_2, \ldots, v_n$, when it beats $v_1$ in the offset mechanism, it is the only such one with constant probability. \jm{What if $v_1$'s noise is uniform between $+\infty$ and $-\infty$? Can be resolved by assuming $v_1$ has no noise, and in the later section we show that's wlog the case we need to consider.}
    \item Therefore, its regret is roughly:
    \[
    \reg(\alg) = \sum_{i = 2}^n \Pr[v_i >_{\alg} v_1] \cdot (v_i - v_1).
    \]
    This is subject to $\sum_{i = 2}^n \Pr[v_i >_{\alg} v_1] \leq 0.5$.
    \item The vector of $v_2, \ldots, v_n$ that minimizes this approximate regret is of interest. The tail bound of Lemma 2 should still hold.
    \item Let the hard instance have $v_1 = 0$. Each of $v_2, \ldots, v_n$ is typically the same as before (maybe with some variance), except that with probability $p_i = \Pr[v_i >_{\alg} v_1]$, it is flipped to the positive $-v_i$. 
    \jm{Define $q_i$ to be the probability that OPT outputs item $i$ when underlying vector is $v$. We should be able to show that this probability is at most $1 - 0.1 \cdot (1 - 10 \cdot q_i)$ when $v_i$ flip to $-v_i$. Therefore the regret from item $i$ is at least $\Omega((q_i + 0.1 \cdot (1 - 10 \cdot q_i)p_i ) (v_1 - v_i)) = \Omega(p_i (v_1 - v_i))$ }
    \item Consider the case where $v_i$ is the unique value in question. No algorithm can distinguish it from $-v_i$ well.
\end{itemize}



\subsection{First item no noise}
Some argument to only look at the case when first item has no noise?

Wlog $v_1 = \arg\max_i v_i$ and 
\begin{align*}
     &\reg(\alg, v) \\
     =& \sum_{i = 2}^n \Pr[v_i +a_i -\theta_i \geq  v_1+a_1 -\theta_1,~ v_i + a_i -\theta_i = \max_{j=2,...,n} v_j + a_j -\theta_j] \cdot (v_1 - v_i) \\
      \leq & \sum_{i = 2}^n \Pr[v_i +a_i -\theta_i \geq  (v_1+v_i)/2,~ v_i + a_i -\theta_i = \max_{j=2,...,n} v_j + a_j -\theta_j] \cdot (v_1 - v_i) \\
      &+\sum_{i = 2}^n \Pr[ (v_1+v_i)/2 \geq  v_1+a_1 -\theta_1,~ v_i + a_i -\theta_i = \max_{j=2,...,n} v_j + a_j -\theta_j] \cdot (v_1 - v_i)\\
      \leq &2\sum_{i = 2}^n \Pr[v_i /2 +a_i -\theta_i \geq  v_1/2,~ v_i/2 + a_i -\theta_i = \max_{j=2,...,n} v_j/2 + a_j -\theta_j] \cdot (v_1/2 - v_i/2) \\
      &+ 2\reg_1\\
\end{align*}

Open question: does our algorithm work for combinatorial optimization e.g. shortest path?


\jm{
It looks like here we can show
\[
\Pr[ a_i \in [\theta_i - v_i^*, \theta_i -1.01\cdot v_i^*]  ] = \Omega( \Pr[a_i \geq \ \theta_i - v_i^*])
\] and
\[
\Pr[ a_i \in [\theta_i + 10 v_i^*, \theta_i - v_i^*]  ] = \Omega(1) \text{  (because }\Pr[a_i < \theta_i + 10 v_i^*] \text{ should be small)}
\]

Suppose we want to make the output distribution $D_i$ for $v_i \sim U[-0.01v_i^*, -0.02 v_i^*]$ (or something similar), and the output distribution $D$ for $v_i \sim U[0.02v_i^*, 0.01 v_i^*]$ to satisfy for some $D_i'$
\[
D > \text{some constant} \cdot \Pr[a_i \geq \ \theta_i - v_i^*] \cdot D_i'
\]
and
\[
D_i > \text{some constant}\cdot D_i'.
\]

And it seems that we just need there exists $k \in  [-0.98, 10]$, 
\[
\Pr[ a_i \in [\theta_i + k \cdot v_i^*, \theta_i + (k-0.01) \cdot v_i^*]]
 = \Omega(1)\]

and it seems that we almost have it.}

\section{Constant-Approximation for $n$ Values}
\subsection{The Offset Algorithm}
Let $A_1, \ldots, A_n$ be the noise distributions. For each $i \in [n]$, choose $\theta_i$ to be the optimal threshold for $A_i$ against $0$, as in the binary-decision setting. This $\theta_i$ satisfies:
\[
\sup_{v_i < 0} \Pr[v_i + a_i > \theta_i] \cdot (-v_i) = \sup_{v_i > 0} \Pr[v_i + a_i < \theta_i] \cdot v_i.
\]

The offset mechanism chooses the value with the largest $v_i + a_i - \theta_i$. We denote this algorithm as $\alg$, and we will show it gives an $O(1)$-approximation in regret against any algorithm. We will use the proved fact that it gives an $s$-approximation for $s = O(1)$ when $n = 2$ and $A_2$ is deterministically $0$.

\subsection{Reduction: Highest Value Has No Noise}
Consider any set of values $\{v_1, \ldots, v_n\}$. Without loss of generality, assume $v_1$ is the largest among them.

Notice that
\begin{align*}
&\reg\big(\alg, (A_1, \ldots, A_n), (v_1, \ldots, v_n)\big)\\
= &\sum_{i = 2}^n \Pr\big[v_i + a_i - \theta_i \geq v_1 + a_1 - \theta_1 \mid v_i + a_i - \theta_i = \max_{j = 2}^n v_j + a_j - \theta_j\big] \cdot (v_1 - v_i)\\
\leq &\sum_{i = 2}^n \bigg(\Pr\big[v_i + a_i - \theta_i \geq \frac{v_1 + v_i}{2} \mid v_i + a_i - \theta_i = \max_{j = 2}^n v_j + a_j - \theta_j\big] \\
&\quad + \Pr\big[\frac{v_1 + v_i}{2} \geq v_1 + a_1 - \theta_1 \mid v_i + a_i - \theta_i = \max_{j = 2}^n v_j + a_j - \theta_j\big]\bigg) \cdot (v_1 - v_i)\\
= &\sum_{i = 2}^n \bigg(\Pr\big[\frac{v_i}{2} + a_i - \theta_i \geq \frac{v_1}{2} \mid v_i + a_i - \theta_i = \max_{j = 2}^n v_j + a_j - \theta_j\big] \\
&\quad + \Pr\big[\frac{v_i}{2} \geq \frac{v_1}{2} + a_1 - \theta_1 \mid v_i + a_i - \theta_i = \max_{j = 2}^n v_j + a_j - \theta_j\big]\bigg) \cdot (v_1 - v_i)\\
\leq &\sum_{i = 2}^n \bigg(\Pr\big[\frac{v_i}{2} + a_i - \theta_i \geq \frac{v_1}{2} \mid \frac{v_i}{2} + a_i - \theta_i = \max_{j = 2}^n \frac{v_j}{2} + a_j - \theta_j\big] \\
&\quad + \Pr\big[\frac{v_i}{2} \geq \frac{v_1}{2} + a_1 - \theta_1 \mid \frac{v_i}{2} = \max_{j = 2}^n \frac{v_j}{2}\big]\bigg) \cdot (v_1 - v_i).
\end{align*}
The first inequality above uses union bound. The second inequality is true since its RHS picks the largest $\frac{v_i}{2} + a_i - \theta_i$ (or $\frac{v_i}{2}$) to compete against $\frac{v_1}{2}$ (or $\frac{v_1}{2} + a_1 - \theta_1$). Further,
\begin{align*}
&\reg\big(\alg, (A_1, \ldots, A_n), (v_1, \ldots, v_n)\big)\\
\leq & \reg(\alg, (0, A_2, \ldots, A_n), (v_1 / 2, v_2 / 2, \ldots, v_n / 2)) + 2 \cdot \reg(\alg, (A_1, 0)).
\end{align*}
Notice that $v_1 / 2$ is still the largest $v_i / 2$. Now we only need to prove
\begin{itemize}
    \item If $v_1$ is the largest in $\alg$, then $\reg(\alg, (0, A_2, \ldots, A_n), (v_1, v_2, \ldots, v_n)) = O(1) \cdot \reg(\opt, (A_1, \ldots, A_n))$.
    \item $\reg(\alg, (A_1, 0)) = O(1) \cdot \reg(\opt, (A_1, \ldots, A_n))$.
\end{itemize}
The second item is immediate, as $\reg(\alg, (A_1, 0)) \leq s \cdot \reg(\opt, (A_1, 0)) \leq s \cdot \reg(\opt, (A_1, A_2)) \leq s \cdot \reg(\opt, (A_1, \ldots, A_n))$. For the first one, we only need that if $v_1$ is the largest among $v_i$'s in $\alg$, then
\[
\reg(\alg, (0, A_2, \ldots, A_n), (v_1, v_2, \ldots, v_n)) = O(1) \cdot \reg(\opt, (0, A_2, \ldots, A_n)).
\]
(This step comes from the fact that $\opt$ can simulate a noise for the first value.) We will be focusing on proving this in the next subsections.

\subsection{Linearization}
Without loss of generality, fix $v_1 = 0$ and impose the constraints that every other $v_i \leq 0$. Let $(v_2^*, \ldots, v_n^*)$ be the solution to maximize
\[
\sum_{i = 2}^n \Pr[v_i + a_i - \theta_i \geq v_1] \cdot (-v_i), \text{\quad  s.t. } \sum_{i = 2}^n \Pr[v_i + a_i - \theta_i \geq v_1] \leq 0.5.
\]
We have
\[
\reg(\alg, (0, A_2, \ldots, A_n)) = \Theta(1) \cdot \reg(\alg, (0, A_2, \ldots, A_n), (0, v_2^*, \ldots, v_n^*)) = \Theta(1) \cdot \sum_{i = 2}^n \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot (-v_i^*).
\]
This is because
\begin{itemize}
    \item $\reg(\alg, (0, A_2, \ldots, A_n)) \geq \reg(\alg, (0, A_2, \ldots, A_n), (0, v_2^*, \ldots, v_n^*))$.
    \item $\reg(\alg, (0, A_2, \ldots, A_n), (0, v_2^*, \ldots, v_n^*)) \geq \frac{1}{2} \cdot \sum_{i = 2}^n \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot (-v_i^*)$, by looking at the case where only one of those $v_i^* + a_i - \theta_i \geq 0$ holds.
    \item (Actually, only this item is useful in the proof.) $\reg(\alg, (0, A_2, \ldots, A_n)) \leq 3 \cdot \sum_{i = 2}^n \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot (-v_i^*)$: We can uniformly and gradually reduce the vector $(v_2, \ldots, v_n)$ that maximizes $\reg(\alg, (0, A_2, \ldots, A_n))$, until $\Pr[\exists i, \ v_i' + a_i - \theta_i \geq 0] \leq \frac{1}{3} < 1 - \frac{1}{\sqrt{e}}$, to get $(v_2', \ldots, v_n')$, losing a factor of at most $3$:
    \begin{align*}
    \reg(\alg, (0, A_2, \ldots, A_n)) &\leq 3 \cdot \reg(\alg, (0, A_2, \ldots, A_n), (v_2', \ldots, v_n'))\\
    &\leq 3 \cdot \sum_{i = 2}^n \Pr[v_i' + a_i - \theta_i \geq 0] \cdot (-v_i')\\
    &\leq 3 \cdot \sum_{i = 2}^n \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot (-v_i^*).
    \end{align*}
\end{itemize}

We therefore only need to prove
\[
\reg(\opt, (0, A_2, \ldots, A_n)) = \Omega(1) \cdot \sum_{i = 2}^n \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot (-v_i^*).
\]

Define $b = \sum_{i = 2}^n \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot (-v_i^*)$. Define $I = \{i \in \{2, 3, \ldots, n\} \mid -v_i^* \geq b\}$. We have
\[
\frac{b}{2} \leq \sum_{i \in I} \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot (-v_i^*) \leq b.
\]
This is because
\begin{align*}
\sum_{i \in I} \Pr[v_i^* + a_i - \theta_i \geq 0] &= b - \sum_{i \in \{2, \ldots, n\} \setminus I} \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot (-v_i^*)\\
&\geq b - \sum_{i \in \{2, \ldots, n\} \setminus I} \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot b \geq 0.5b.
\end{align*}


\subsection{Case (1): Some $i \in I$ Satisfies $\Pr[a_i \in [\theta_i - 0.5 v_i^*, \theta_i - v_i^*]] \geq 0.2$}
In this case, we have
\begin{align*}
\reg(\opt, (0, A_2, \ldots, A_n)) &\geq \reg(\opt, (0, A_i), (0, 0.5v_i^*))\\
&\geq \frac{1}{s} \cdot \reg(\alg, (0, A_i), (0, 0.5v_i^*))\\
&= \frac{1}{s} \cdot \Pr[0.5v_i^* + a_i > \theta_i] \cdot (-0.5 v_i^*)\\
&\geq \frac{0.1}{s} \cdot (-v_i^*) \geq \frac{0.1}{s} \cdot b.
\end{align*}

\subsection{Case (2): No $i \in I$ Satisfies $\Pr[a_i \in [\theta_i - 0.5 v_i^*, \theta_i - v_i^*]] \geq 0.2$}
\begin{lemma}
For any $\lambda > 1$, $\Pr[a_i \geq \theta_i - \lambda \cdot v_i^* \mid a_i \geq \theta_i - v_i^*] \leq \frac{1}{\lambda}$.
\end{lemma}
\begin{proof}
It comes from the optimality of $v_i^*$. Replacing it with $\lambda v_i^*$ is still feasible, and thus should not improve the objective.
\end{proof}

\begin{lemma}
$\Pr[a_i \in [\theta_i - v_i^*, \theta_i -1.1\cdot v_i^*]] \geq 0.09 \cdot \Pr[a_i \geq \ \theta_i - v_i^*]$.
\end{lemma}
\begin{proof}
Just use the previous lemma.
\end{proof}

\begin{lemma}
$\Pr[a_i \in [\theta_i + 5 v_i^*, \theta_i - 0.5v_i^*]] \geq 0.1$.
\end{lemma}
\begin{proof}
Firstly, $\Pr[a_i > \theta_i - v_i^*] \leq 0.5$ by the choice of $v_i^*$ (we have $\sum_{i \in \{2, \ldots, n\}} \Pr[a_i > \theta_i - v_i^*] \leq 0.5$).

Next, notice that $\Pr[a_i < \theta_i + 5v_i^*] \leq 0.2$ by the choice of $\theta_i$. Otherwise, $\Pr[-5v_i^* + a_i < \theta_i] > 0.2$, giving a regret of more than $-v_i^*$ if it is against a zero-noise value. However, for negative values, the regret is less than $-v_i^*$ by the optimality of $v_i^*$. However, $\theta_i$ should have balanced the regrets instead.

Finally, $\Pr[a_i \in [\theta_i - 0.5v_i^*, \theta_i - v_i^*]] < 0.2$ by the case condition.
\end{proof}

\begin{lemma}
There exists some $k_i \in [-0.4, 5]$, so that
\[
\Pr[a_i \in [\theta_i + k_i \cdot v_i^*, \theta_i + (k_i-0.1) \cdot v_i^*]] \geq \frac{1}{550}.
\]
\end{lemma}
\begin{proof}
This is from the Pigeonhole principle.
\end{proof}

\begin{lemma}
For the distribution $v_i \sim U[1.2 \cdot v_i^*, v_i^*]$, $v_i + a$ covers $0.045 \cdot \Pr[a_i \geq \theta_i - v_i^*]$ fraction in probability of $U[\theta_i + 0.1v_i^*, \theta_i]$.
\end{lemma}
\begin{proof}
Fix any $w \in [\theta_i + 0.1v_i^*, \theta_i]$. We have
\begin{align*}
f(t) &= \int_{1.2 \cdot v_i^*}^{v_i^*} \frac{1}{0.2 v_i^*} \cdot f_{A_i}(w - v_i) \d v_i\\
&\geq \int_{w - \theta_i + 1.1 \cdot v_i^*}^{w - \theta_i + v_i^*} \frac{1}{0.2 v_i^*} \cdot f_{A_i}(w - v_i) \d v_i\\
&= \frac{1}{0.2 v_i^*} \cdot \int_{\theta_i - v_i^*}^{\theta_i - 1.1 \cdot v_i^*} f_{A_i}(a_i) \d a_i\\
&\geq \frac{1}{0.2 v_i^*} \cdot 0.09 \cdot \Pr[a_i \geq \theta_i - v_i^*]\\
&\geq \frac{1}{0.1 v_i^*} \cdot 0.045 \cdot \Pr[a_i \geq \theta_i - v_i^*]. \qedhere
\end{align*}
\end{proof}

\begin{lemma}
For the distribution $v_i \sim U[(-k_i + 0.2) \cdot v_i^*, (-k_i) \cdot v_i^*]$, $v_i + a$ covers $0.0009$ fraction in probability of $U[\theta_i + 0.1v_i^*, \theta_i]$.
\end{lemma}
\begin{proof}
Similar to the lemma above.
\end{proof}

Now consider the following hard instance for $\opt$:
\begin{itemize}
    \item $v_1$ is known to be $0$.
    \item $v_i$ is``typically'' drawn from $U[0.4 \cdot v_i^*, 0.2 \cdot v_i^*]$. ($v_i^* \leq 0.2 v_i^*$ in this case.)
    \item With probability $\Pr[v_i^* + a_i - \theta_i \geq 0]$ in a disjoint way, $v_i$ is instead ``atypically'' drawn from $U[(-k_i - 0.6) \cdot v_i^*, (-k_i - 0.8) \cdot v_i^*]$. ($v_i^* \geq -0.2 \cdot v_i^*$ in this case.)
\end{itemize}

\begin{lemma}
$\reg(\opt, (0, A_2, \ldots, A_n)) \geq 1.8 \times 10^{-4} \cdot \sum_{i \in I} \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot (-v_i^*)$ for the instance above.
\end{lemma}
\begin{proof}
Let $p_i$ be the probability that $\opt$ chooses $v_i$ conditioned on the instance being ``typical''. Let $q_i$ be the probability that $\opt$ chooses $v_i$ conditioned on $v_i$ being ``atypical''. We have
\[
\reg(\opt, (0, A_2, \ldots, A_n)) \geq \sum_{i \in I} \left(\frac{1}{2} \cdot p_i \cdot (-0.2v_i^*) + \Pr[v_i^* + a_i - \theta_i \geq 0] \cdot (1 - q_i) \cdot (-0.2v_i^*)\right).
\]
Let $r_i$ be the probability of $\opt$ picking $v_i$ if $v_i \sim U[\theta_i - 0.7v_i^*, \theta_i - 0.8v_i^*]$. We have
\[
p_i \geq r_i \cdot 0.045 \cdot \Pr[a_i \geq \theta_i - v_i^*], \text{ and } 1 - q_i \geq (1 - r_i) \cdot 0.0009.
\]
Therefore,
\begin{align*}
\reg(\opt, (0, A_2, \ldots, A_n)) &\geq \sum_{i \in I} \left(\frac{1}{2} \cdot r_i \cdot 0.045 \cdot (-0.2v_i^*) + (1 - r_i) \cdot 0.0009 \cdot (-0.2v_i^*)\right) \cdot \Pr[a_i \geq \theta_i - v_i^*]\\
&\geq 1.8 \times 10^{-4} \cdot \sum_{i \in I} \Pr[a_i \geq \theta_i - v_i^*] \cdot (-v_i^*). \qedhere
\end{align*}
\end{proof}

To summarize, we have the following theorem:
\begin{theorem}
The offset algorithm gives a $20000$-approximation in regret for the $n$ value case against any algorithm.
\end{theorem}

\section{Other Results}
\begin{itemize}
\item Picking the item with the best expectation is not a constant-approximation, even for $2$ items.
\item Possible generalization to picking $k$ items? Graph problems such as shortest path? Revenue maximization?
\end{itemize}

An obstacle to $k$-item generalization is that the noise for $k$ i.i.d. bounded random variables will concentrate as $k \to \infty$. Todo: calculate this.
